Configuration Learning in Underwater Optical Links

A new research problem named configuration learning is described in this work. A novel algorithm is proposed to address the configuration learning problem. The configuration learning problem is defined to be the optimization of the Machine Learning (ML) classifier to maximize the ML performance metric optimizing the transmitter configuration in the signal processing/communication systems. Specifically, this configuration learning problem is investigated in an underwater optical communication system with signal processing performance metric of the physical-layer communication throughput. A novel algorithm is proposed to perform the configuration learning by alternating optimization of key design parameters and switching between several Recurrent Neural Network (RNN) classifiers dependant on the learning objective. The proposed ML algorithm is validated with the datasets of an underwater optical communication system and is compared with competing ML algorithms. Performance results indicate that the proposal outperforms the competing algorithms for binary and multi-class configuration learning in underwater optical communication datasets. The proposed configuration learning framework can be further investigated and applied to a broad range of topics in signal processing and communications.

==> comment.tex <==
% The benefit of the proposal is that neither Signal-to-Noise Ratio~(SNR) nor Channel State Information~(CSI) measurements are required at the receiver to perform configuration learning.
% With the trained classifier deployed at the receiver, the system is able to perform 
% Therefore, the proposal is suited for those systems with no interface to acquire SNR and/or CSI information. 

% The criterion in the LSTM classifier is to minimize the square loss of the predicted label number and the trained label number. 
% The proposed machine learning algorithm firstly performs a Fourier Transform to filter the out-of-band noise, then performs a Walsh-Hadamard transform to reduce the signal dimensionality. The transform-domain tensor is send to the LSTM for training.
% A framework on configuration learning is proposed for the physical-layer adaptation of underwater optical links with the configuration classified by deep neural network. The proposed framework is investigated on an underwater wireless optical communication system with range-extension capabilities realized by the structures of the large-scale photodetector array and time-frequency spreading. The configuration learning classifier is chosen to be Long Short-Term Memory~(LSTM)-based Recurrent Neural Network~(RNN) classifier. The training data is chosen to be the pre-detection signal at the communication receiver. The objective of the configuration-learning classifier is to determine the optimal transmitter configuration that maximizes the physical-layer throughput based on the pre-detection signal. This work is the first investigation of the physical-layer configuration learning by LSTM-based RNN classifier. The physical-layer throughput performance results and the received pre-detection signal datasets are generated by a link-level simulator that emulates the hardware system performance in the realistic underwater optical channel. The classifiers under comparison include decision tree, adaptive boosting ensemble classifier, and random subspace ensemble classifier. Results indicate that the LSTM-based RNN classifier outperforms all classifiers under comparison, and can successfully achieves zero classification error with reasonable complexity. Results further verify that the training datasets of the pre-detection signal achieve much better performance than the post-detection signal. The proposed configuration-learning framework by deep recurrent neural network has broad applications in communication link adaptation. 
%
% The results datasets include the time-frequency spreading and coding rate specifications that achieve the highest physical-layer throughput, given a set of parameters including the distance/signal-to-noise ratio, and the AUV moving speed. The machine learning classifiers are tested with the objective of classifying binary-class or multi-class system configurations with the inputs of distance/signal-to-noise ratio and the AUV moving speed. Classification results of k-fold cross-validation successfully indicate that, for binary-class system configurations, the ensemble classifiers can achieve high classification accuracy; while for three-class system configurations, the decision tree classifier can achieve high classification accuracy. However, the classification for different channel coding rate is still difficult for the machine learning classifiers. To address this technical challenge, further evaluations are performed on LSTM-based RNN deep learning classifier. The datasets for training are tested for the amplitude of the signals at the input or output of MRC. It is found by classification results that, the datasets chosen to be the input of MRC has achieved good classification for three classes and six classes, including the classification of the different coding rates. Therefore the LSTM-based RNN deep learning classifier based on pre-signal-detection datasets can successfully solve the classification problem for different channel coding rate, therefore is the well-suited machine learning algorithm for the system adaptation classification.

% The physical optical channel modeling follows the experimentally-verified models to closely emulate the physical optical channel including the simulations in this work are based on the physical-layer simulator with the transceiver signal processing chain.

% depending on the feature set of the configuration learning, and the alternating optimization of the parameter of the switched ML classifier.


% \item System design and link-level simulation: Optical large-scale photodetector and time-frequency spreading are deployed to improve the coverage range. Optical communication system design is proposed and the link-level simulation is performed to obtain the frame error rate and physical-layer throughput results. The results indicate that the proposed structure can effectively improve the coverage by several folds for simulation setups of different autonomous underwater vehicles~(AUV) transmitter speed, coding rate and spreading parameters. The link-level simulator is built on realistic physical-layer channel models and includes signal processing blocks in both transmitter and receiver.

% \item Configuration learning: The physical-layer throughput datasets are generated for the proposed system for different AUV speed and distances. Based on the datasets, multiple classes are identified as the classification objective. A number of machine learning classifiers are tested on the datasets. It is found that, for binary classification, LSTM based recurrent neural network classifier with training data chosen as pre-detection signal, can achieve zero classification error for training cycle greater than 14; while for three-class and six-class classification, LSTM based recurrent neural network classifier with training of pre-detection signal can achieve zero classification error for training cycle greater than 18. These performance results outperform the decision tree and adaptive boosting ensemble classifier under comparison.
% }


% This proposal is especially well-suited for hardware systems without interface for acquiring SNR and/or CSI information. 

% 
% The deep learning is applied to channel estimation in wireless communication systems~\cite{He18} and to recover Channel State Information~(CSI) from reduced-sized codewords~\cite{Wen18}. There are general discussions of deep learning in wireless systems~\cite{Wang19}. 

% 
% The existing works on deep learning based physical-layer communication system design are mostly on the detection of data symbols and on channel estimation at the receiver. The conventional neural networks are applied to the detection of data symbols~\cite{Shea17} where the communication system is modeled by an autoencoder. The similar structure of deep learning based signal detector has been described~\cite{Wang17} for both symbol detection and decoding. A Sliding Bidirectional Recurrent Neural Network (SBRNN) is proposed~\cite{Farsad18} to detect the symbol streams in the communication receiver. 

% In Sect.~\ref{sec:related}, the related works are summarized.

% 
% In subsect.\ref{sec:datasets}, the dataset generation method is described for the training of the machine learning classifiers.

% % Other existing proposals adopt Multiple Input Multiple Output~(MIMO) and Orthogonal Frequency Division Multiplexing~(OFDM) techniques, including a MIMO-OFDM acoustic system~\cite{Baosheng09} achieving $125.7~\rm{kbit/s}$ communication rate over a bandwidth of $62.5~\mathrm{kHz}$, a MIMO-OFDM system~\cite{Nelson14} for underwater communications using 4-by-4 MIMO, acoustic MIMO~\cite{Bouvet14,Martins14}, acoustic MIMO space-time coding techniques~\cite{Zorita15}, and acoustic MIMO coded modulation~\cite{Pelekanakis11}. 

% \item System design and simulation: Based on the channel characteristics as well as on the properties of the laser and on the sampling rate of ADC/DAC, an OFDM-based optical communication design is proposed and the structure is validated with the link-level simulator built to emulate the physical-layer performance of the practical hardware system;

% ---------------------------------------------------------------
% --------------------------------------------------------------

% \section{Related Works}\label{sec:related}

% On the design and realization of underwater optical systems, an OFDM-based underwater optical communication system is implemented in~\cite{Hessien18} based on a variation of LTE frame structure and OFDM parameters. An underwater wireless optical communication system with $100~\rm{Mbps}$ and full-duplex function is implemented in~\cite{Li18} with $520~\rm{nm}$ laser diodes for two pairs of single-transmitter and single-receiver setups. A sea trial of underwater optical communication with a two-channel MIMO approach is presented in~\cite{Scholz18}, and coverage range and packet loss were analyzed. Bit Error Rate~(BER) and changes in the scintillation index of blue, green, and red laser beams through turbulence-induced underwater channels are evaluated in~\cite{Oubei18}. The performances of the Blue Ray modem and alternative modulation schemes are analyzed in~\cite{Herji18}. An OFDM-based Multiuser-MIMO system for underwater visible light communication is introduced in~\cite{Amantayeva18}, with a 2-by-2 MIMO system and $532~\rm{nm}$ LED transmitters. A pre-coding pulse amplitude modulation technique is proposed in~\cite{Shi18} to mitigate the effect of the nonlinearity of electrical-to-optical conversion in the optical source. The analytical performance of underwater optical communication is studied in~\cite{Elamassie18}, and the relay-based structure is described considering detect-and-forward and amplify-and-forward relays. In existing works, there is no OFDM here is no massive MIMO and time-frequency spreading though, and the coverage of the system is not described. 

% There are related works on underwater optical sensor network~\cite{Saeed18}, where a multi-hop sensor network is studied on the network localization, and an optimization problem is formulated and solved by the conjugate gradient method.

% A distributed energy-efficient and balanced routing algorithm is presented in~\cite{Liu18}, where each sensor node only knows its own position and the locations of sink nodes so that broadcasting for topology discovery is avoided to save batteries. A general software-defined networking structure for optical wireless communication is describe in~\cite{Shahjalal18}, where the control functionality is separated from the data plane. A robust 3D localization method to improve the localization accuracy for underwater optical wireless sensor networks is proposed in~\cite{Saeed2018}, where a low-rank matrix approximation method is employed for estimating inter-node distances.

% ---------------------------------------------------------------
% -------------------------------------------------------------

% \\ \hline
% $s_{n} (j)$      & The constellation symbol before time-frequency spreading at transmitter, $n = 1,...,N_{TX}$ and $j = 1,...,N_{TFS}$. 
% \\ \hline
% $x_{n}(k,i)$      & The spread symbol after time-frequency spreading at transmitter, $k = 1,...,N_{SUBC}$, $i = 1,...,N_{OFDM}$. 
% \\ \hline
% $r_{m}(k,i)$      & Received signal before the signal detector at the receiver, $m = 1,...,N_{RX}$.
% \\ \hline
% $y_{n}(k,i)$      & The detected spread symbol before time-frequency de-spreading at receiver.
% \\ \hline
% $a_l(j)$      & The spread sequence of length $L = N_T N_F$ for the $j$-th constellation symbol, $l = 1,...,L$.
% \\ \hline
% $v_{n}(j)$      & The constellation symbol after time-frequency de-spreading at receiver. 
% \\ \hline
% $h_{n,m}(k,i)$      & Channel response between the transmitter and the receiver in frequency domain.
% \\ \hline
% $\hat h_{n,m}(k,i)$      & Channel estimation output at the receiver.


% It is found by data analysis that the LSTM-based RNN classifier achieves the best possible classification accuracy performance; therefore it is chosen as the ML classifier in the proposal.

% The rationale that LSTM-based RNN performs very well can be explained based on the similarities between the data sequence received at the communication receiver and the datasets of Natural Language Processing~(NLP) speech sequence. First, the communication channel changes the signal strength and causes time-domain variations of the received signal. The time-sequences of speech datasets also have signal strength and time-domain variations. Second, the communication channel introduces noise in the received data sequence. This effect is similar to the speech data where the environmental and recording noise is presented in the dataset. Furthermore, the datasets of received signals are sequential datasets that have correlations in the data, similar to the speech data sequences. LSTM-based RNN is the widely accepted ML method for NLP applications including speech recognition. LSTM-based RNN is well-suited for the application of classifying large sequential data, which is also the case of our configuration classification problem.

% \subsection{Dataset Generation for Training of the Machine Learning Classifiers}\label{sec:datasets}

% \begin{tabular}{l|l|l|l}
% \hline
% \begin{tabular}[c]{@{}l@{}}Variable AUV Speed
% \end{tabular} & 
% \begin{tabular}[c]{@{}l@{}}Variable Distance\end{tabular} &  
% \begin{tabular}[c]{@{}l@{}}ML Feature Vector\end{tabular}  & 
% \begin{tabular}[c]{@{}l@{}}ML Label\end{tabular}\\ 
% \hline
% AUV speed \#1: $0.1~\rm{m/s}$      & \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}\small{For each AUV speed:}\\ \small{60 AUV-Buoy distances}\\\small{1m to 60m, spacing 1m}\\\small{Totally 240 machine}\\\small{learning samples}\end{tabular}} & \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}\small{For each ML sample:}\\ \small{Vector of 128 complex numbers}\\ \small{32 per OFDM symbol multiplied}\\ \small{by 4 receiving photodetector}\end{tabular}} & \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}\small{For each ML sample:}\\\small{The coding and spreading}\\\small{configuration maximizing the}\\ \small{physical-layer throughput}\end{tabular}} \\ 
% \cline{1-1}
% AUV speed \#2: $0.3~\rm{m/s}$   &   &                                                                                                                                                       &  \\ \cline{1-1}
% AUV speed \#3: $0.4~\rm{m/s}$   &                                                                                                  &                                                                                                                                                            &                                                                                                                                                        \\ \cline{1-1}
% AUV speed \#4: $0.5~\rm{m/s}$       &                                                                                                                                           & &   \\ \hline
% Generated dataset size     &     & \begin{tabular}[c]{@{}l@{}}\small{240 samples of feature vector}\end{tabular}       & \begin{tabular}[c]{@{}l@{}}\small{240 samples of label}\end{tabular}  \\ \hline
% \end{tabular}

% \centering
% \\begin{center}
%\vspace{-0.4cm}
% \includegraphics[width=0.53\textwidth]{fig/Table_Data.pdf}
% \end{center}
% \vspace{-0.5cm}

% For the LSTM-based RNN, the results of accuracy with the number of hidden units are generated. Based on a comprehensive data analysis, the LSTM-based RNN classifier achieves the best performance among the ML classifiers evaluated. Therefore in this work of configuration classification, the LSTM-based RNN classifier is chosen as the classifier at the receiver to determine the transmitter specification. These results are also consistent with ML works on NLP dataset classification, where LSTM achieves improvements compared with other approaches in classifying the sequential datasets.


% The LSTM classifier is based on the criterion of minimizing the square error of the predicted label number and the training label number. The criterion is designed in the training process of the stochastic gradient descent algorithm. In the proposed algorithm, this criterion is realized in the LSTM classifier. The modulation and coding schemes are labeled by integer numbers and the training algorithm in LSTM is to minimize the square error. The reason that LSTM can perform better than competing machine learning algorithm is, the LSTM has the improved modeling of the internal structure of the neural cells. 

% The trained LSTM-based RNN classifier is deployed at the receiver. The received signal is sent to the LSTM-based RNN classifier for the online classification. The classified optimal configuration is sent to the transmitter via feedback signalling link to adjust the transmitter specification.

% The training dataset design is based on the observations that, the key features of the channel are preserved in the data $r_m (k,i)$. In contrast, the post-detection signal $y_n^{} (k,i)$ does not contain the information of channel amplitude gain, due to the equalization by the signal detector. This observation is further verified by the latter simulation results that, the classification accuracy of the post-detection signal $y_n^{} (k,i)$ is much less than the pre-detection signal. 


% \subsection{Large-Scale Photodetector Array and Time-Frequency Spreading Structure}\label{sec:propse:array}

% In our proposal, a large-scale photodetector array is deployed at the receiver and the time-frequency spreading is performed at the transmitter. The communication coverage can be greatly improved by these two approaches, indicated by the link-level simulation results.

% The underwater optical system with one single photodetector at the receiver suffers attenuation even at very short distances. 

%The received signal at the OFDM demodulation output can be written by
%\begin{equation}
%r_m^{} (k,i) = h_{n,m}^{} (k,i) \cdot x_n^{} (k,i) + n_m^{} (k,i)
%\end{equation}
%In our system, the signals $x_{n,m}^{} (k,i)$ at the transmitter LED sources $n = 1,...,N_{TX}$ can be spatial multiplexed signal, where the number of data streams equals to $N_{TX}$.
%
%With large-scale photodetector array, the $N_{RX}$ is a large number up to a few hundred. The system model can be written in matrix format by
%\begin{equation}
%{\bf{r}}(k,i) = {\bf{H}}(k,i) \cdot {\bf{x}}(k,i) + {\bf{n}}(k,i)
%\end{equation}
%where ${\bf{r}}(k,i)$ is the received signal vector of size $N_{RX}$-by-1; {\bf{H}}(k,i) is the channel matrix of size $N_{RX}$-by-$N_{TX}$; ${\bf{x}}(k,i)$ is the transmitted signal vector of size $N_{TX}$-by-1; and ${\bf{n}}(k,i)$ is the Additive White Gaussian Noise~(AWGN) noise vector of size $N_{RX}$-by-1.
%The zero-forcing signal detection can be deployed at the receiver to recovery the transmitted signal by
%\begin{equation}
%{\bf{y}}(k,i) = \left[ {{\bf{\hat H}}^H (k,i){ \bf{\hat H}}(k,i)} \right]_{}^{ - 1} {\bf{\hat H}}^H (k,i) \cdot {\bf{r}}(k,i)
%\end{equation}
%where ${\bf{\hat H}}$ is the channel estimatino matrix composed of the channel estimates $\hat h_{n,m}(k,i)$.
%
%The spreading is done at the transmitter, where the constellation symbol $s_n^{} (j)$ is spread by the spreading sequence $a_l(j)$ of length $L$ by
%\begin{equation}
%{\bf{\tilde s}}_n (j) = s_n^{} (j){\bf{a}}_n^{} (j)
%\end{equation}
%where ${\bf{\tilde s}}_n (j)$ is $j$-th the spread signal vector at the $n$-th spatial stream. ${\bf{\tilde s}}_n (j)$ is of length $L$-by-1. This signal is further mapped to the $N_T$-by-$N_F$ time-frequency subcarrier allocations and the allocated signal is represented by $x_n (k,i)$, where $k = 1,...,N_F$, and $i= 1,...,N_T$.
%The de-spreading procedure is performed at the receiver to recover the signal $v_n(j)$ with the signal detector output ${y}(k,i)$. The time-frequency spread can improve the SNR by a factor of $L$. The SNR improvement by zero-forcing detection depends on the channel realizations. Given large-scale photodetector array, the physical-layer simulation results in the following sections indicate that the system can achieve notable coverage extension by several folds with the receiver large-scale photodetector array design.

% }


%{
% We illustrate now our proposed system in detail, including our novel contributions, i.e., the adoption of a large-scale photodetector array at the receiver and a Time-Frequency~(TF) spreading at the transmitter (Sect.~\ref{sec:propse:array}). The LSTM-based recurrent neural network is reviewed (Sect.~\ref{sec:review:LSTM}), and the proposed classifier for the configuration learning problem is presented with the explanations of the training procedure. 
% (Sect.~\ref{sec:propse:LSTM}).
% }

% What about Sect.~\ref{sec:propse:capa}? 
%
% Based on rigorous analyses, we derive the formula of the theoretical data rate with the combination of the large-scale photodetector array and TF-spreading. Note that the receiver sensitivity is enhanced by the adoption of a large-scale photodetector array. With the maximum ratio combining at the receiver, the SNR is significantly improved. 


% For the optical system, the multipath propagation characteristic has  scattering effect causing a very small multipath delay of maximum $10~\rm{ns}$, thus introducing Inter Symbol Interference~(ISI). We have designed the OFDM system with the Cyclic Prefix~(CP) to mitigate this ISI effect. The linear modulation of the OFDM optical signal can be realized by tuning of the laser beam photonic density. 

% \begin{figure*}
% \begin{minipage}[ht]{0.5\linewidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/FER_01.eps}
%  \begin{center} 
%  (a)
%  \end{center}
%  \end{minipage}% 
%  \begin{minipage}[ht]{0.5\linewidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/01ms_1_100.eps}
%  \begin{center} 
%  (b)
%  \end{center}
%  \end{minipage}% 
%  \caption{Performance of 1-by-100 system with an AUV speed of $0.1~\rm{m/s}$: (a)~Frame error rate; (b)~Physical-layer throughput.}\label{fig 0.1}
% \end{figure*}

% \begin{figure*}
% \begin{minipage}[ht]{0.5\linewidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/FER_03.eps}
%  \begin{center} 
%  (a)
%  \end{center}
%  \end{minipage}% 
%  \begin{minipage}[ht]{0.5\linewidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/03ms_1_100.eps}
%  \begin{center} 
%  (b)
%  \end{center}
%  \end{minipage}% 
%  \caption{Performance of 1-by-100 system with an AUV speed of $0.3~\rm{m/s}$: (a)~Frame error rate; (b)~Physical-layer throughput.}\label{fig 0.3}
% \end{figure*}


% \begin{figure*}
% \begin{minipage}[ht]{0.5\linewidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/FER_05.eps}
%  \begin{center} 
%  (a)
%  \end{center}
%  \end{minipage}% 
%  \begin{minipage}[ht]{0.5\linewidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/05ms_1_100.eps}
%  \begin{center} 
%  (b)
%  \end{center}
%  \end{minipage}% 
%  \caption{Performance of 1-by-100 system with an AUV speed of $0.5~\rm{m/s}$: (a)~Frame error rate; (b)~Physical-layer throughput.}\label{fig 0.5}
% \end{figure*}


% On the optical noise model related parameters, the following values are chosen: scalar irradiance of the solar light $\Phi$ is $0.8109~\rm{W/m^2}$; the receiving aperture area $A_r$ is $0.01~\rm{m^2}$; the transmit power $P_T$ is $50~\rm{W}$; the receiver sensitivity $\gamma_0$ is $0.5~\rm{A/W}$; the combined efficiency of the transmitter and receiver $\eta_0$ is $0.81$; the inclination angle $\beta_0$ is chosen to be $0$ degree; the diverge angle of the transmitter $\theta$ is $68$ degrees; the attenuation coefficient $c$ is $0.1514~\rm{m^{-1}}$; the photocurrent parameter $I_L$ is $100$; the temperature is $290~\rm{K}$; the load resistance is $100~\rm{\Omega}$; the photodiode parameter $I_D$ is $1.226 \times 10^{-9}$.

% \begin{figure*}[t]
%   \begin{minipage}[ht]{0.33\linewidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/lstm_hidden_all.eps}
%  \begin{center} 
%  (a)
%  \end{center}
%  \end{minipage}% 
%  \begin{minipage}[ht]{0.33\linewidth} 
%  \centering
%  \includegraphics[width=\textwidth]{fig/bilstm_hidden_all.eps}
%  \begin{center}
%  (b) 
%  \end{center} 
%  \end{minipage}
%  \begin{minipage}[ht]{0.33\linewidth} 
%  \centering
%  \includegraphics[width=\textwidth]{fig/gru_hidden_all.eps}
%  \begin{center}
%  (c) 
%  \end{center} 
%  \end{minipage}
 
% \caption{Accuracy  of  classifiers  vs  number  of  hidden  units: (a) LSTM-based RNN classifier; (b) bi-directional LSTM classifier; (c)  GRU classifier.
% }\label{fig ML classifier vs numhid}
%  \end{figure*}

% (a), when the AUV speed is $0.1~\rm{m/s}$, for single-input system with QPSK modulation and a code rate of 1/2, the coverage is $21~\rm{m}$ for 1-by-100 system without spreading, $30~\rm{m}$ for 1-by-100 system with $N_F = 16$ and $N_T = 1$. By adding the time-domain spreading, the coverage is further improved: $34~\rm{m}$ for 1-by-100 system with $N_F = 16$ and $N_T = 8$. It is found that the time-domain spreading can further improve the coverage on top of the frequency-domain spreading. In Fig.~\ref{fig SIMO TF FER}(d), when the AUV speed is $0.5~\rm{m/s}$, for the single-photonic transmitter system with QPSK modulation and a code rate of 1/3, the coverage is $7~\rm{m}$ for 1-by-100 system without spreading because of the low SNR. The coverage is $20~\rm{m}$ for 1-by-100 system with the frequency-domain spreading of $N_F = 16$ and time-domain spreading of $N_T = 1$, which increase the coverage three times compared with that of 1-by-100 system without spreading. After adding time-domain spreading, the coverage increases to $26~\rm{m}$ for 1-by-100 system with frequency-domain spreading of $N_F = 16$ and time-domain spreading of $N_T = 8$. From this plot, it can be observed that the time-domain spreading can achieve improved performance to mitigate the Doppler effect. 


% \begin{figure*}[t]
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/lstm_2.eps}
% \label{fig: lstm2}
% \begin{center} 
% (a)
% \end{center}
% \end{minipage}% 
% \begin{minipage}[t]{0.5\linewidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/lstm_36.eps}
% \label{fig: lstm36}
%  \begin{center} 
%  (a)
%  \end{center}
%  \end{minipage}% 
%  \caption{Training classification error convergence curve of LSTM-based RNN classifier {\color{red}with $600$ hidden units} for (a) binary classification and (b) multi-class classification. }\label{fig:LSTM}
% \end{figure*}

% \begin{figure*}[t]
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/bilstm_2.eps}
% \label{fig: lstm2}
% \begin{center} 
% (a)
% \end{center}
% \end{minipage}% 
% \begin{minipage}[t]{0.5\linewidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/bilstm_36.eps}
% \label{fig: lstm36}
%  \begin{center} 
%  (a)
%  \end{center}
%  \end{minipage}% 
%  \caption{\color{red}Training classification error convergence curve of bi-directional LSTM classifier {\color{red}with $600$ hidden units} for (a) binary classification and (b) multi-class classification. }\label{fig:BiLSTM}
% \end{figure*}

% \begin{figure*}[t]
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/gru_2.eps}
% \label{fig: lstm2}
% \begin{center} 
% (a)
% \end{center}
% \end{minipage}% 
% \begin{minipage}[t]{0.5\linewidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/gru_36.eps}
% \label{fig: lstm36}
%  \begin{center} 
%  (a)
%  \end{center}
%  \end{minipage}% 
%  \caption{\color{red}Training classification error convergence curve of GRU classifier {\color{red}with $600$ hidden units} for (a) binary classification and (b) multi-class classification. }\label{fig:GRU}
% \end{figure*}

% \begin{figure*}[t]
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/dt_2.eps}
% \label{fig: dt2}
% \begin{center} 
% (a)
% \end{center}
% \end{minipage}% 
% \begin{minipage}[t]{0.5\linewidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/dt_36.eps}
%  \label{fig: dt36}
%  \begin{center} 
%  (a)
%  \end{center}
%  \end{minipage}% 
%  \caption{Training classification error convergence curve of decision tree classifier for (a) binary classification and (b) multi-class classification. }\label{fig:Decision_Tree}
% \end{figure*}

% For $0.3~\rm{m/s}$ AUV speed and one transmitting source, where the Doppler shift is $1.32 \times 10^5~\rm{Hz}$, the coverage distance is improved to $21~\rm{m}$ with a throughput of $100~\rm{Mbps}$ by 1-by-100 system with $1/3$ Turbo code, to $28~\rm{m}$ with a throughput of $4~\rm{Mbps}$ by 1-by-100 system with frequency spreading and $1/3$ Turbo code, and to $33~\rm{m}$ with a throughput of $700~\rm{kbps}$ by 1-by-100 system with time-frequency spreading and $1/2$ Turbo code.
% For $0.4~\rm{m/s}$ AUV speed and one transmitting source, where the Doppler shift is $1.76 \times 10^5~\rm{Hz}$, the coverage distance is improved to $18~\rm{m}$ with a throughput of $100~\rm{Mbps}$ by 1-by-100 system with $1/3$ Turbo code, to $26~\rm{m}$ with a throughput of $4~\rm{Mbps}$ by 1-by-100 system with frequency spreading and $1/3$ Turbo code, and to $31~\rm{m}$ with a throughput of $700~\rm{kbps}$ by 1-by-100 system with time-frequency spreading and $1/2$ Turbo code.


% \begin{figure*}[t]
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/abe2.eps}
%  \label{fig: abe2}
% \begin{center} 
% (a)
% \end{center}
% \end{minipage}% 
% \begin{minipage}[t]{0.5\linewidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/abe_36.eps}
%  \label{fig: abe36}
%  \begin{center} 
%  (a)
%  \end{center}
%  \end{minipage}% 
%  \caption{Training classification error convergence curve of adaptive boosting ensemble classifier for (a) binary classification and (b) multi-class classification. }\label{fig:AdaBoost}
% \end{figure*}

% \begin{figure*}[t]
% \begin{minipage}[t]{0.33\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/lstm_2.eps}
% \begin{center}
% (a)
% \end{center}
% \end{minipage}%
% \begin{minipage}[t]{0.33\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/dt_2.eps}
% \begin{center}
% (b)
% \end{center}
% \end{minipage}%
% \begin{minipage}[t]{0.33\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/abe2.eps}
% \begin{center}
% (c)
% \end{center}
% \end{minipage}
% % \begin{minipage}[t]{0.5\linewidth}
% % \centering
% % \includegraphics[width=\textwidth]{fig/rse_2.eps}
% % \begin{center}
% % (d)
% % \end{center}
% % \end{minipage}%
% \caption{{ Accuracy} of different methods of machine learning for binary classification with training by pre-detection signal: (a)~LSTM-based RNN classifier; (b)~Decision tree; (c)~Adaptive boosting ensemble.
% % ; (d) Random subspace ensemble. 
% }\label{fig: two class}
% % \vspace{-0.7cm}
% \end{figure*}


% \begin{figure*}[t]
% \begin{minipage}[t]{0.33\linewidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/lstm_36.eps}
%  \begin{center} 
%  (a)
%  \end{center}
%  \end{minipage}% 
% \begin{minipage}[t]{0.33\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/dt_36.eps}
% \begin{center}
% (b)
% \end{center}
% \end{minipage}%
%     \begin{minipage}[t]{0.33\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/abe_36.eps}
% \begin{center}
% (c)
% \end{center}
% \end{minipage}
% % \begin{minipage}[t]{0.5\linewidth}
% % \centering
% % \includegraphics[width=\textwidth]{fig/rse_36.eps}
% % \begin{center}
% % (d)
% % \end{center}
% % \end{minipage}
% \caption{ { Accuracy} of different methods of machine learning for multi-class classification with training by pre-detection signal: (a)~LSTM-based RNN classifier; (b)~Decision tree; (c)~Adaptive boosting ensemble.
% % ; (d) Random subspace ensemble. 
% % \vspace{-0.7cm}
% }\label{fig: six class}
% \end{figure*}

% \begin{figure}[t]
%  \centering
%     \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/LSTM_B.eps}
% \begin{center}
% (a)
% \end{center}
% \end{minipage}%
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/LSTM.eps}
% \begin{center}
% (b)
% \end{center}
% \end{minipage}%

% \centering
%     \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/TREE_B.eps}
% \begin{center}
% (c)
% \end{center}
% \end{minipage}%
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/TREE.eps}
% \begin{center}
% (d)
% \end{center}
% \end{minipage}%

% \caption{ Classification error of Different methods of machine learning for binary classification: (a) LSTM-based RNN classifier  training by pre-detection signal; (b) LSTM-based RNN classifier training by post-detection signal; (c) Decision tree training by pre-detection signal; (d) Decision tree training by post-detection signal.}\label{fig: two class: tree vs LSTM}
% \end{figure}
%
%\begin{figure}[t]
%  \centering
%    \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/LSTM_B6.eps}
% \begin{center}
% (a)
% \end{center}
% \end{minipage}%
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/LSTM6.eps}
% \begin{center}
% (b)
% \end{center}
% \end{minipage}%
%
%\centering
%    \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/TREE_B6.eps}
% \begin{center}
% (c)
% \end{center}
% \end{minipage}%
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/TREE6.eps}
% \begin{center}
% (d)
% \end{center}
% \end{minipage}%
%
%  \caption{Classification error of Different methods of machine learning for multi-class classification: (a) LSTM-based RNN classifier training by pre-detection signal; (b) LSTM-based RNN classifier training by post-detection signal; (c) Decision tree training by pre-detection signal; (d) Decision tree training by post-detection signal.}\label{fig: six class: tree vs LSTM}
%\end{figure}


% \begin{figure*}[t]
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/numHid_2class.eps}
% \begin{center} 
% (a)
% \end{center}
% \end{minipage}% 
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/numHid_6class.eps}
% \begin{center} 
% (b)
% \end{center}
%  \end{minipage}% 
%  \caption{{Accuracy} of LSTM vs number of hidden units {\color{red} with $50$ epochs}: (a)~Binary classification; (b)~Multiple-class classification.}\label{fig: numHiddenUnit}
%  \vspace{-0.7cm}
% \end{figure*}

% \begin{figure*}[t]
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/bilstm_hidden2.eps}
% \begin{center} 
% (a)
% \end{center}
% \end{minipage}% 
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/bilstm_hidden36.eps}
% \begin{center} 
% (b)
% \end{center}
%  \end{minipage}% 
%  \caption{{Accuracy} of bi-directional LSTM vs number of hidden units {\color{red} with $50$ epochs}: (a)~Binary classification; (b)~Multiple-class classification.}\label{fig: bilstm_numHiddenUnit}
%  \vspace{-0.7cm}
% \end{figure*}

% \begin{figure*}[t]
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/gru_hidden2.eps}
% \begin{center} 
% (a)
% \end{center}
% \end{minipage}% 
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=\textwidth]{fig/gru_hidden36.eps}
% \begin{center} 
% (b)
% \end{center}
%  \end{minipage}% 
%  \caption{{Accuracy} of GRU vs number of hidden units {\color{red} with $50$ epochs}: (a)~Binary classification; (b)~Multiple-class classification.}\label{fig: gru_numHiddenUnit}
%  \vspace{-0.7cm}
% \end{figure*}

